Controlling Diversity at Inference: Guiding Diffusion Recommender Models with Targeted Category Preferences

Diversity control is an important task to alleviate bias amplification and filter bubble problems. The desired degree of diversity may fluctuate based on users' daily moods or business strategies. However, existing methods for controlling diversity often lack flexibility, as diversity is decided during training and cannot be easily modified during inference. We propose \textbf{D3Rec} (\underline{D}isentangled \underline{D}iffusion model for \underline{D}iversified \underline{Rec}ommendation), an end-to-end method that controls the accuracy-diversity trade-off at inference. D3Rec meets our three desiderata by (1) generating recommendations based on category preferences, (2) controlling category preferences during the inference phase, and (3) adapting to arbitrary targeted category preferences. In the forward process, D3Rec removes category preferences lurking in user interactions by adding noises. Then, in the reverse process, D3Rec generates recommendations through denoising steps while reflecting desired category preferences. Extensive experiments on real-world and synthetic datasets validate the effectiveness of D3Rec in controlling diversity at inference.

==> tables/5exp_hyper_noise.tex <==
% Second Table
\begin{table}[t]
\caption{Effect of the noise scale $s$ on Steam dataset.}
 \vspace{+0.1cm}
 \resizebox{\linewidth}{!}{
\begin{tabular}{c|cccc}
\toprule
Noise scale & Recall@20 & NDCG@20 & Entropy@20 & Coverage@20 \\
\midrule
$10^{-3}$ & 0.063 & 0.052 & 0.768 & 0.805 \\
$10^{-2}$ & 0.066 & 0.054 & 0.762 & \textbf{0.810} \\
$10^{-1}$ & 0.067 & 0.055 & 0.769 & 0.803 \\
1    & \textbf{0.069} & \textbf{0.056} & \textbf{0.771} & 0.805 \\
\bottomrule
\end{tabular}}
\label{tab:hyper_noise}
\end{table}

==> tmp_sentence.tex <==

Systems with restricted controllability run the risk of diminishing user satisfaction \cite{control_satis}.
However, these systems fail to provide adequate user control \cite{control_survey} and are susceptible to bias amplification due to the uneven distribution of item categories (e.g., movie genres) in users' historical data \cite{Calib, DecRs}.


Among efforts to break the filter bubbles, there is a growing focus in recommendation systems that provide a set of diverse items.\cite{DCRS, DGRec}.
Also, some works \cite{FDSB, DCRS} have demonstrated through an online A/B test that augmenting the diversity of recommended items led to increased user engagement.
Existing methods to diversify the recommended items are divided into two main strategies: the post-processing \cite{DPP, ComiRec, FDSB} and the end-to-end \cite{DPGNN, DGCN, DPCML} approaches.
In the initial stage of diversified recommendation \cite{DiRec, MMR, ER, PPTM}, a post-processing module designed for enhancing diversity is introduced after generating candidates.
Since the post-processing module works independently of candidate generation, this strategy is separated from the optimization of the relevance matching module.
As the diversity signal is not reflected in the accuracy promotion process, there is an increased risk that the final recommended outcome may be suboptimal \cite{DGCN}.
This issue is well known as the accuracy and diversity dilemma \cite{dilemma}.
To address this dilemma, end-to-end approaches \cite{DGCN, DGRec, DCRS, DPCML, DPGNN} have been proposed, which jointly optimize relevance and diversity during training.
Most methods alleviate the dilemma by utilizing item category information, focusing primarily on recommending items from categories that users have rarely consumed yet have some history with.
However, the integration of diversity signals has resulted in losing its ability to control over the balance between accuracy and diversity.
If users desire less or more diverse recommendations, they must either provide user feedback or adjust the parameters that balance accuracy and diversity, requiring retraining the model.
This process of accommodating changing user preferences is inefficient and inappropriate, potentially diminishing user satisfaction.



To tackle these challenges, we first conduct causal reasoning and analyze the causal factors influencing the interaction generation procedure, which are depicted in Figure \ref{fig:causal} as a causal graph.
Since the user interaction $\boldsymbol{x}$ intrinsically contains information about the category preferences $\boldsymbol{y}$, as shown in Figure \ref{fig:causal} (a), the user representation $\boldsymbol{z}$, which could be obtained by Conditional Variational Autoencoders (CVAEs) \cite{vae, csvae, pcvae, COR}, includes conflicting information from $\boldsymbol{y}$ and $\tilde{\boldsymbol{y}}$, degrading generation quality.
To address this adverse impact, we adopt a diffusion framework \cite{DDPM}.
By adding noise to the interaction, we eliminate the preference information embedded within and predict the user's interaction through denoising while reflecting $\tilde{\boldsymbol{y}}$.
Moreover, to reflect the diversity in a fine-grained manner with category preference, we leverage disentanglement.
